Personalized Video Summarization by Multimodal Video Understanding

Video summarization techniques have been proven to improve the overall user experience when it comes to accessing and comprehending video content. If the user's preference is known, video summarization can identify significant information or relevant content from an input video, aiding them in obtaining the necessary information or determining their interest in watching the original video. Adapting video summarization to various types of video and user preferences requires significant training data and expensive human labeling. To facilitate such research, we proposed a new benchmark for video summarization that captures various user preferences. Also, we present a pipeline called Video Summarization with Language (VSL) for user-preferred video summarization that is based on pre-trained visual language models (VLMs) to avoid the need to train a video summarization system on a large training dataset. The pipeline takes both video and closed captioning as input and performs semantic analysis at the scene level by converting video frames into text. Subsequently, the user's genre preference was used as the basis for selecting the pertinent textual scenes. The experimental results demonstrate that our proposed pipeline outperforms current state-of-the-art unsupervised video summarization models. We show that our method is more adaptable across different datasets compared to supervised query-based video summarization models. In the end, the runtime analysis demonstrates that our pipeline is more suitable for practical use when scaling up the number of user preferences and videos.

==> tables/SSTV/SSTV_SOTA.tex <==

\begin{table*}
    \centering
    \scriptsize
    \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{l|cccccc|cccccc|cccccc}
    \toprule
         TV show & \multicolumn{6}{c|}{pbs kids} & \multicolumn{6}{c|}{modern marvel} & \multicolumn{6}{c}{house cut}\\
         \midrule
         Genre & \multicolumn{2}{c}{general} & \multicolumn{2}{c}{children-talk} & \multicolumn{2}{c|}{anime} & \multicolumn{2}{c}{general} & \multicolumn{2}{c}{documentary} & \multicolumn{2}{c|}{cookie} & \multicolumn{2}{c}{general} & \multicolumn{2}{c}{children} & \multicolumn{2}{c}{house} \\
         \midrule
          Target length & $1/3$ & $1/6$ & $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$ \\
         \midrule
         Current pipeline (video) &   &   &   &&& &0.316 &0.274 &  & & & &0.295& 0.302&   &   &  &   \\
         Current pipeline (text) &   &   &   &&&&  & &  0.481 &0.340 &0.534&0.414&&& 0.414 & 0.370 & 0.403 & 0.458 \\
        \midrule
        MomentDETR (scene) & 0.378 & 0.231 & 0.405 & 0.226 & 0.377 & 0.259 & 0.350 & 0.200 & 0.338 & 0.192& 0.474& 0.244 & 0.383 & 0.359 & 0.357 & 0.262 & 0.333 & 0.347 \\ 
        MomentDETR & 0.378 & 0.231 & 0.405 & 0.226 & 0.377 & 0.259 & 0.375 & 0.234 & 0.451 & 0.221& 0.462& 0.213 & 0.355 & 0.137 & 0.296 & 0.196 & 0.426 & 0.192 \\ 
        QD-DETR \cite{} &  0.440 & 0.249  & 0.385  & 0.230  & 0.431  & 0.331  & 0.364  & 0.266  & 0.480  & 0.331 & 0.495 &  0.303 & 0.332 & 0.182 & 0.296 & 0.213 & 0.326 & 0.159 \\ 
        UniVTG \cite{lin2023univtg} &  0.411 & 0.371  & 0.474  & 0.342  & 0.307  & 0.193  & 0.432  & 0.305  & 0.542  & 0.344 & 0.402 &  0.257 & 0.325 & 0.167 & 0.248 & 0.167 & 0.354 & 0.144 \\ 
        A2Sum &  &  &  &&&&& &  &&&&&&& \\
    \bottomrule    
    \end{tabular}
    }
    \caption{Samsung TV Plus video summarization SOTA models. Reported by averaged $F_1$.}
    \label{tab:sota}
\end{table*}

==> tables/SSTV/SSTV_dialog_coherient.tex <==

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{c|ccc}
         Method & pbs kids & modern marvel & house cut\\
         \hline
        MomentDETR &   &  & \\
        A2Sum &  &  & \\
        QD-DETR &  &  & \\
    \end{tabular}
    \caption{Samsung TV Plus dialog coherent. Reported by ?.}
    \label{tab:my_label}
\end{table}

==> tables/SSTV/SSTV_query.tex <==


\begin{table*}
    \centering
    \scriptsize
    \resizebox{2\columnwidth}{!}{%
    \begin{tabular}{l|cccccc|cccccc|cccccc}
         TV show & \multicolumn{6}{c|}{pbs kids} & \multicolumn{6}{c|}{modern marvel} & \multicolumn{6}{c}{house cut}\\
         \hline
         Genre & \multicolumn{2}{c}{general} & \multicolumn{2}{c}{children-talk} & \multicolumn{2}{c|}{anime} & \multicolumn{2}{c}{general} & \multicolumn{2}{c}{documentary} & \multicolumn{2}{c|}{cookie} & \multicolumn{2}{c}{general} & \multicolumn{2}{c}{children} & \multicolumn{2}{c}{house} \\
         \hline
          Target length & $1/3$ & $1/6$ & $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$& $1/3$ & $1/6$ \\
         \hline
        MomentDETR & 0.378 & 0.231 & 0.405 & 0.226 & 0.377 & 0.259 & 0.375 & 0.234 & 0.451 & 0.221& 0.462& 0.213 & 0.355 & 0.137 & 0.296 & 0.196 & 0.426 & 0.192 \\ 
        Genre &  &  &  &&&&& & 0.395 & 0.348 & 0.516& 0.409 &&&& \\
        ASR summary &  &&  &&&&& &  &&&&&&&&\\
        Caption summary &  &&  &&&&& &  &&&&&&&&\\
    \end{tabular}
    }
    \caption{Samsung TV Plus with different types of queries. Reported by $F_1$.}
    \label{tab:diff_query}
\end{table*}

% \begin{table*}
%     \centering
%     \scriptsize
%     \begin{tabular}{c|ccc|ccc|ccc}
%          \multirow{2}{*}{Method} & \multicolumn{3}{c|}{pbs kids} & \multicolumn{3}{c|}{modern marvel} & \multicolumn{3}{c}{house cut}\\
%          & general& children-talk & anime &general &documentary& cookie&general&children & house\\
%          \hline
%         TV show title & 0.581 & 0.531 & 0.394& &&& 0.559 & 0.599& 0.621\\
%         TV show title + genre&   &   &  & &&&   &  &  \\
%         ASR summary &  & &&&&&& & \\
%         Caption summary &  & &&&&&& & \\
%     \end{tabular}
%     \caption{Samsung TV Plus with different types of queries. Reported by $F_1$.}
%     \label{tab:my_label}
% \end{table*}

==> tables/dataset_comparison.tex <==

\begin{table*}[t!]
\setlength{\tabcolsep}{0.15em}
\small
\centering
\caption{Comparison with existing moment retrieval datasets. Our proposed data aims to capture high-level semantics given the genre queries. Also, each genre query will be mapped to multiple moments (scenes).}
%\resizebox{\textwidth}{!}{
\begin{tabular}{p{3.2cm}
P{1.8cm}
P{2.2cm}
P{1.6cm}P{2.2cm}P{2.0cm}}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Domain} & \multirow{2}{*}{\#Queries/\#Videos}   & Avg & Avg Len (sec) & Avg \#Moments  \\
 &  &  & Query Len  & Moment/Video & per Query  \\ 
\midrule
DiDeMo~\cite{anne2017localizing} & Flickr & 41.2K / 10.6K & 8.0 & 6.5 / 29.3  & 1 \\
ANetCaptions~\cite{Krishna2017DenseCaptioningEI} & Activity & 72K / 15K  & 14.8 & 36.2 / 117.6  & 1  \\
CharadesSTA~\cite{gao2017tall} & Activity & 16.1K / 6.7K  & 7.2 & 8.1 / 30.6 & 1  \\
TVR~\cite{lei2020tvr} & TV show & 109K / 21.8K & 13.4 & 9.1 / 76.2 & 1   \\
How2R \cite{li2020hero} & Instructional & 51K/24K & 18 & 15 / 60 & 1   \\
QVHighlight \cite{momentdetr}& Vlog / News & 10.3K / 10.2K  & 11.3 & 24.6 / 150 & 1.8  \\
mTVR \cite{lei2021mtvr}&  TV show & 218K / 21.8K  & 13.4 &  9.1 / 76.2 & 1  \\
\midrule
\DatasetName & Movie & 1.8K / 1K  & 1 & 3 / 180 & 9   \\
\bottomrule
\end{tabular}
%}
\label{tab:dset_comparison}
\end{table*}


% \begin{table*}[t!]
% \setlength{\tabcolsep}{0.15em}
% \small
% \centering
% \caption{Comparison with existing moment retrieval (\textit{top}) and highlight detection (\textit{bottom}) datasets. \textit{Q}=\textit{Query}, \textit{MR}=\textit{Moment Retrieval}, \textit{HD}=\textit{Highlight Detection}.}
% \begin{tabular}{p{3.2cm}
% P{1.8cm}
% P{2.2cm}
% P{1.6cm}P{2.2cm}P{2.0cm}P{1.2cm}P{1.2cm}P{0.9cm}}
% \toprule
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Domain} & \multirow{2}{*}{\#Queries/\#Videos}   & Avg & Avg Len (sec) & Avg \#Moments  & \multicolumn{2}{c}{Supported Tasks} & Has \\
%  &  &  & Query Len  & Moment/Video & per Query & MR & HD & Query \\ 
% \midrule
% DiDeMo~\cite{anne2017localizing} & Flickr & 41.2K / 10.6K & 8.0 & 6.5 / 29.3  & 1 &  \cmark & - & \cmark \\
% ANetCaptions~\cite{Krishna2017DenseCaptioningEI} & Activity & 72K / 15K  & 14.8 & 36.2 / 117.6  & 1 & \cmark & - & \cmark \\
% CharadesSTA~\cite{gao2017tall} & Activity & 16.1K / 6.7K  & 7.2 & 8.1 / 30.6 & 1 & \cmark & - & \cmark \\
% TVR~\cite{lei2020tvr} & TV show & 109K / 21.8K & 13.4 & 9.1 / 76.2 & 1 & \cmark & - & \cmark  \\
% QVHighlight \cite{momentdetr}& Vlog / News & 10.3K / 10.2K  & 11.3 & 24.6 / 150 & 1.8 & \cmark & \cmark & \cmark  \\
% \midrule
% MoveiGenreSum & Movie & 1.8K / 1K  & 1 & 2.5 / 150 & 2.2 & \cmark & \cmark & \cmark  \\
% \bottomrule
% \end{tabular}
% \label{tab:dset_comparison}
% \end{table*}

==> tables/multi_length.tex <==
\begin{table}[h]
\centering
\resizebox{.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}}& \textbf{Video Summarization}& \multicolumn{3}{c}{Summarization length} \\
 \cmidrule(l){3-5}  
 &\textbf{Training Data}& short & medium & long \\
\midrule
MomentDETR \cite{momentdetr} &QV-highlight& 14.3 & 26.0 & 50.2 \\
QD-DETR \cite{qddetr} &QV-highlight& 14.4 & 26.1 & 50.3 \\
UniVTG \cite{lin2023univtg} &10 Datasets& 15.2 & 26.1 & 51.3 \\
\midrule
ZVSL & - & 19.3 & 29.4 & 52.3  \\
\bottomrule
\end{tabular}}
%}
\vspace{5mm}
\caption{Multi-length video summarization. Evaluated by F1 score.}
\label{genre}
\end{table}

